Using CEF Digital Service Infrastructures in the Smart4Health Project for the Exchange of Electronic Health Records

The Smart4Health (S4H) software application will empower EU citizens to manage, analyze, and exchange their aggregated electronic health data. In order to provide such a service, basic features are needed to ensure usability, reliability, and trust. The CEF building blocks implement such functionalities while complying with EU regulations. This report examines the current status and applicability of the CEF building blocks for the envisioned S4H software application. The major findings of the report are that (1) most CEF building blocks are currently not ready to be applied without further implementation efforts and (2) the S4H-specific use cases and user needs, to which the single CEF building blocks correspond, must be clarified. Open questions raised in this report need to be answered before a clear analysis can be made. Moreover, the functionalities of CEF building blocks aim at the matured product, while for the first version of the S4H software application basic implementations suffice. Still, concepts need to be elaborated of how the sample implementation of CEF building blocks or suitable alternative applications can be included into the system at a later point.

==> chapters/CEF_DSIs/eHealth_Use_Cases.tex <==
\subsection{eHealth}

S4H will not implement functionalities already incorporated in the eHDSI, such as the Patient Summary and ePrescription, but rather use the defined data structures and include collected medical information. Therefore, the NCPs developed as part of the eHDSI play an important role as a data source. How the communication between S4H and NCPs will be established needs to be discussed; one possibility is to connect the NCPs to the ingestion pipeline and/or to use eDelivery.

Additionally, the terminology services could be included to ensure a proper translation of medication and other nation-specific terms.

However, since the implementation of eHealth relies on other components, it will not be further discussed in \autoref{sec:implementation}.
